Stubborn Set Reduction for Two-Player Reachability Games

Partial order reductions have been successfully applied to model checking of concurrent systems and practical applications of the technique show nontrivial reduction in the size of the explored state space. We present a theory of partial order reduction based on stubborn sets in the game-theoretical setting of 2-player games with reachability objectives. Our stubborn reduction allows us to prune the interleaving behaviour of both players in the game, and we formally prove its correctness on the class of games played on general labelled transition systems. We then instantiate the framework to the class of weighted Petri net games with inhibitor arcs and provide its efficient implementation in the model checker TAPAAL. Finally, we evaluate our stubborn reduction on several case studies and demonstrate its efficiency.

==> sections/resulttable-full.tex <==
\section{Full Result Table}\label{sec:allresults}
%\begin{table}[t]
%\centering
%\scalebox{1}{
\begin{longtable}{|l|r|r|r|r|r|r|}
\hline
& \multicolumn{2}{c|}{Time (seconds)} &\multicolumn{2}{c|}{Markings $\times1000$} & \multicolumn{2}{c|}{Reduction}  \\\hline
Model& NORMAL & POR & NORMAL & POR& \%Time & \%Markings \\\hline\hline
AIM-1-50-3-1&0.0&0.0&1&0&0&100\\\hline
AIM-1-50-3-11&0.0&0.1&10&9&0&10\\\hline
AIM-1-50-3-16&0.1&0.1&15&15&0&0\\\hline
AIM-1-50-3-21&0.1&0.1&20&20&0&0\\\hline
AIM-1-50-3-6&0.0&0.0&5&4&0&20\\\hline
AIM-1-50-6-1&0.0&0.0&1&0&0&100\\\hline
AIM-1-50-6-11&0.1&0.1&11&7&0&36\\\hline
AIM-1-50-6-16&0.1&0.1&16&11&0&31\\\hline
AIM-1-50-6-21&0.1&0.1&19&14&0&26\\\hline
AIM-1-50-6-6&0.0&0.0&5&4&0&20\\\hline
AIM-1-50-9-1&0.0&0.0&1&0&0&100\\\hline
AIM-1-50-9-11&0.1&0.1&10&10&0&0\\\hline
AIM-1-50-9-16&0.1&0.1&15&15&0&0\\\hline
AIM-1-50-9-21&0.1&0.1&18&19&0&-6\\\hline
AIM-1-50-9-6&0.0&0.0&4&4&0&0\\\hline
AIM-1-50-12-1&0.0&0.0&1&0&0&100\\\hline
AIM-1-50-12-11&0.1&0.1&11&7&0&36\\\hline
AIM-1-50-12-16&0.1&0.1&15&11&0&27\\\hline
AIM-1-50-12-21&0.1&0.1&20&14&0&30\\\hline
AIM-1-50-12-6&0.0&0.0&6&4&0&33\\\hline
AIM-1-100-3-1&0.0&0.0&1&1&0&0\\\hline
AIM-1-100-3-11&0.1&0.2&21&15&-100&29\\\hline
AIM-1-100-3-16&0.2&0.3&31&22&-50&29\\\hline
AIM-1-100-3-21&0.3&0.3&41&29&0&29\\\hline
AIM-1-100-3-6&0.1&0.1&11&8&0&27\\\hline
AIM-1-100-6-1&0.0&0.0&1&1&0&0\\\hline
AIM-1-100-6-11&0.2&0.2&21&15&0&29\\\hline
AIM-1-100-6-16&0.2&0.3&30&21&-50&30\\\hline
AIM-1-100-6-21&0.3&0.3&41&28&0&32\\\hline
AIM-1-100-6-6&0.1&0.1&11&8&0&27\\\hline
AIM-1-100-9-1&0.0&0.0&1&1&0&0\\\hline
AIM-1-100-9-11&0.2&0.2&21&15&0&29\\\hline
AIM-1-100-9-16&0.2&0.3&30&21&-50&30\\\hline
AIM-1-100-9-21&0.3&0.3&40&28&0&30\\\hline
AIM-1-100-9-6&0.1&0.1&10&7&0&30\\\hline
AIM-1-100-12-1&0.0&0.0&1&1&0&0\\\hline
AIM-1-100-12-11&0.2&0.2&21&15&0&29\\\hline
AIM-1-100-12-16&0.2&0.3&31&22&-50&29\\\hline
AIM-1-100-12-21&0.3&0.4&39&27&-33&31\\\hline
AIM-1-100-12-6&0.1&0.1&10&7&0&30\\\hline
AIM-1-150-12-1&0.0&0.0&2&1&0&50\\\hline
AIM-1-150-12-11&0.3&0.4&31&30&-33&3\\\hline
AIM-1-150-12-16&0.5&0.6&46&47&-20&-2\\\hline
AIM-1-150-12-21&0.6&0.8&61&61&-33&0\\\hline
AIM-1-150-12-6&0.2&0.2&16&14&0&12\\\hline
AIM-1-150-3-1&0.0&0.0&2&1&0&50\\\hline
AIM-1-150-3-11&0.3&0.3&31&24&0&23\\\hline
AIM-1-150-3-16&0.5&0.5&46&37&0&20\\\hline
AIM-1-150-3-21&0.6&0.7&61&51&-17&16\\\hline
AIM-1-150-3-6&0.2&0.2&16&12&0&25\\\hline
AIM-1-150-6-1&0.0&0.0&2&1&0&50\\\hline
AIM-1-150-6-11&0.3&0.4&31&26&-33&16\\\hline
AIM-1-150-6-16&0.4&0.5&46&41&-25&11\\\hline
AIM-1-150-6-21&0.6&0.6&60&58&0&3\\\hline
AIM-1-150-6-6&0.2&0.2&16&13&0&19\\\hline
AIM-1-150-9-1&0.0&0.0&2&1&0&50\\\hline
AIM-1-150-9-11&0.3&0.4&31&28&-33&10\\\hline
AIM-1-150-9-16&0.4&0.5&46&45&-25&2\\\hline
AIM-1-150-9-21&0.6&0.8&61&61&-33&0\\\hline
AIM-1-150-9-6&0.2&0.2&16&13&0&19\\\hline
AIM-3-50-12-1&0.0&0.0&5&2&0&60\\\hline
AIM-3-50-12-11&0.9&0.6&64&32&33&50\\\hline
AIM-3-50-12-16&1.2&0.7&93&46&42&51\\\hline
AIM-3-50-12-21&1.5&0.9&122&61&40&50\\\hline
AIM-3-50-12-6&0.4&0.3&35&17&25&51\\\hline
AIM-3-50-3-1&0.0&0.0&5&3&0&40\\\hline
AIM-3-50-3-11&0.7&0.6&59&45&14&24\\\hline
AIM-3-50-3-16&1.1&0.9&85&74&18&13\\\hline
AIM-3-50-3-21&1.4&1.2&113&99&14&12\\\hline
AIM-3-50-3-6&0.4&0.3&32&21&25&34\\\hline
AIM-3-50-6-1&0.0&0.0&5&2&0&60\\\hline
AIM-3-50-6-11&0.8&0.6&61&31&25&49\\\hline
AIM-3-50-6-16&1.2&0.8&89&46&33&48\\\hline
AIM-3-50-6-21&1.3&0.9&113&59&31&48\\\hline
AIM-3-50-6-6&0.4&0.3&32&17&25&47\\\hline
AIM-3-50-9-1&0.0&0.0&5&3&0&40\\\hline
AIM-3-50-9-11&0.7&0.7&60&53&0&12\\\hline
AIM-3-50-9-16&1.1&0.9&86&79&18&8\\\hline
AIM-3-50-9-21&1.5&1.2&109&102&20&6\\\hline
AIM-3-50-9-6&0.3&0.4&28&27&-33&4\\\hline
AIM-3-100-12-1&0.1&0.1&10&5&0&50\\\hline
AIM-3-100-12-11&2.1&1.6&122&62&24&49\\\hline
AIM-3-100-12-16&3.1&2.3&177&91&26&49\\\hline
AIM-3-100-12-21&4.1&2.7&226&119&34&47\\\hline
AIM-3-100-12-6&1.2&0.9&64&33&25&48\\\hline
AIM-3-100-3-1&0.2&0.1&9&5&50&44\\\hline
AIM-3-100-3-11&2.3&1.6&118&63&30&47\\\hline
AIM-3-100-3-16&3.5&2.1&172&92&40&47\\\hline
AIM-3-100-3-21&3.9&3.0&227&121&23&47\\\hline
AIM-3-100-3-6&1.3&0.9&64&34&31&47\\\hline
AIM-3-100-6-1&0.2&0.1&9&5&50&44\\\hline
AIM-3-100-6-11&2.3&1.6&117&62&30&47\\\hline
AIM-3-100-6-16&3.0&2.1&171&90&30&47\\\hline
AIM-3-100-6-21&4.4&2.7&226&119&39&47\\\hline
AIM-3-100-6-6&1.2&0.9&63&33&25&48\\\hline
AIM-3-100-9-1&0.2&0.1&10&5&50&50\\\hline
AIM-3-100-9-11&2.3&1.8&121&63&22&48\\\hline
AIM-3-100-9-16&3.5&2.4&173&92&31&47\\\hline
AIM-3-100-9-21&4.6&3.4&231&121&26&48\\\hline
AIM-3-100-9-6&1.2&0.9&62&34&25&45\\\hline
AIM-3-150-12-1&0.3&0.3&14&8&0&43\\\hline
AIM-3-150-12-11&4.9&4.5&177&148&8&16\\\hline
AIM-3-150-12-16&6.7&7.0&261&230&-4&12\\\hline
AIM-3-150-12-21&7.9&8.0&343&302&-1&12\\\hline
AIM-3-150-12-6&2.1&2.3&95&67&-10&29\\\hline
AIM-3-150-3-1&0.3&0.3&14&8&0&43\\\hline
AIM-3-150-3-11&4.0&3.6&175&108&10&38\\\hline
AIM-3-150-3-16&5.7&5.2&254&166&9&35\\\hline
AIM-3-150-3-21&7.3&6.2&336&230&15&32\\\hline
AIM-3-150-3-6&2.5&1.9&94&55&24&41\\\hline
AIM-3-150-6-1&0.3&0.3&14&8&0&43\\\hline
AIM-3-150-6-11&4.6&4.0&174&120&13&31\\\hline
AIM-3-150-6-16&5.9&5.7&255&192&3&25\\\hline
AIM-3-150-6-21&8.5&6.9&334&275&19&18\\\hline
AIM-3-150-6-6&2.6&2.0&94&58&23&38\\\hline
AIM-3-150-9-1&0.3&0.3&14&8&0&43\\\hline
AIM-3-150-9-11&4.5&3.9&176&134&13&24\\\hline
AIM-3-150-9-16&5.8&6.5&256&220&-12&14\\\hline
AIM-3-150-9-21&7.8&6.2&340&298&21&12\\\hline
AIM-3-150-9-6&2.5&1.6&95&63&36&34\\\hline
AIM-5-50-12-1&0.2&0.1&15&5&50&67\\\hline
AIM-5-50-12-11&2.6&1.5&161&59&42&63\\\hline
AIM-5-50-12-16&4.0&1.6&233&86&60&63\\\hline
AIM-5-50-12-21&4.8&2.3&306&113&52&63\\\hline
AIM-5-50-12-6&1.6&0.7&88&32&56&64\\\hline
AIM-5-50-3-1&0.2&0.1&13&6&50&54\\\hline
AIM-5-50-3-11&2.6&1.9&144&97&27&33\\\hline
AIM-5-50-3-16&3.4&3.0&209&163&12&22\\\hline
AIM-5-50-3-21&4.9&3.4&275&221&31&20\\\hline
AIM-5-50-3-6&1.5&0.9&78&44&40&44\\\hline
AIM-5-50-6-1&0.2&0.1&13&5&50&62\\\hline
AIM-5-50-6-11&2.6&1.4&150&57&46&62\\\hline
AIM-5-50-6-16&4.1&2.0&218&83&51&62\\\hline
AIM-5-50-6-21&4.6&2.7&281&109&41&61\\\hline
AIM-5-50-6-6&1.5&0.7&80&31&53&61\\\hline
AIM-5-50-9-1&0.2&0.1&13&8&50&38\\\hline
AIM-5-50-9-11&2.7&2.1&149&122&22&18\\\hline
AIM-5-50-9-16&4.1&3.6&213&181&12&15\\\hline
AIM-5-50-9-21&4.8&4.0&274&235&17&14\\\hline
AIM-5-50-9-6&1.3&1.2&74&62&8&16\\\hline
AIM-5-100-12-1&0.7&0.4&27&10&43&63\\\hline
AIM-5-100-12-11&9.3&4.6&300&115&51&62\\\hline
AIM-5-100-12-16&13.0&6.0&436&168&54&61\\\hline
AIM-5-100-12-21&15.2&8.7&561&219&43&61\\\hline
AIM-5-100-12-6&4.7&2.5&160&62&47&61\\\hline
AIM-5-100-3-1&0.6&0.4&26&10&33&62\\\hline
AIM-5-100-3-11&8.2&4.5&288&116&45&60\\\hline
AIM-5-100-3-16&10.7&6.2&419&169&42&60\\\hline
AIM-5-100-3-21&12.7&7.5&552&222&41&60\\\hline
AIM-5-100-3-6&4.2&2.5&157&63&40&60\\\hline
AIM-5-100-6-1&0.6&0.3&25&9&50&64\\\hline
AIM-5-100-6-11&8.8&4.4&288&113&50&61\\\hline
AIM-5-100-6-16&11.9&5.7&417&164&52&61\\\hline
AIM-5-100-6-21&14.4&7.4&551&216&49&61\\\hline
AIM-5-100-6-6&4.8&2.4&157&61&50&61\\\hline
AIM-5-100-9-1&0.7&0.4&27&10&43&63\\\hline
AIM-5-100-9-11&8.0&4.7&299&117&41&61\\\hline
AIM-5-100-9-16&11.8&6.7&429&170&43&60\\\hline
AIM-5-100-9-21&16.9&7.7&568&224&54&61\\\hline
AIM-5-100-9-6&5.0&2.5&158&63&50&60\\\hline
AIM-5-150-12-11&17.2&12.3&436&321&28&26\\\hline
AIM-5-150-12-1&1.4&0.9&39&17&36&56\\\hline
AIM-5-150-12-16&22.9&18.4&638&505&20&21\\\hline
AIM-5-150-12-21&30.0&23.5&836&663&22&21\\\hline
AIM-5-150-12-6&9.9&6.7&237&140&32&41\\\hline
AIM-5-150-3-11&17.2&10.1&427&211&41&51\\\hline
AIM-5-150-3-1&1.3&0.6&38&16&54&58\\\hline
AIM-5-150-3-16&25.2&14.8&619&330&41&47\\\hline
AIM-5-150-3-21&28.8&17.6&815&464&39&43\\\hline
AIM-5-150-3-6&9.6&5.5&232&106&43&54\\\hline
AIM-5-150-6-11&17.9&10.5&425&244&41&43\\\hline
AIM-5-150-6-1&1.3&0.8&38&15&38&61\\\hline
AIM-5-150-6-16&25.5&15.4&620&402&40&35\\\hline
AIM-5-150-6-21&29.7&22.4&812&589&25&27\\\hline
AIM-5-150-6-6&10.0&5.8&231&115&42&50\\\hline
AIM-5-150-9-11&17.2&12.7&431&283&26&34\\\hline
AIM-5-150-9-1&1.3&0.8&38&16&38&58\\\hline
AIM-5-150-9-16&20.2&19.6&626&479&3&23\\\hline
AIM-5-150-9-21&27.6&23.1&826&651&16&21\\\hline
AIM-5-150-9-6&9.0&5.5&235&128&39&46\\\hline
AIM-7-50-12-1&0.6&0.2&29&9&67&69\\\hline
AIM-7-50-12-11&7.6&2.6&301&98&66&67\\\hline
AIM-7-50-12-16&9.8&4.3&436&143&56&67\\\hline
AIM-7-50-12-21&12.0&4.9&571&188&59&67\\\hline
AIM-7-50-12-6&3.8&1.6&166&54&58&67\\\hline
AIM-7-50-3-1&0.5&0.3&25&11&40&56\\\hline
AIM-7-50-3-11&6.1&4.0&266&168&34&37\\\hline
AIM-7-50-3-16&8.1&6.7&385&286&17&26\\\hline
AIM-7-50-3-21&10.6&9.6&507&387&9&24\\\hline
AIM-7-50-3-6&3.7&2.0&146&76&46&48\\\hline
AIM-7-50-6-1&0.5&0.2&26&8&60&69\\\hline
AIM-7-50-6-11&7.2&2.7&278&95&62&66\\\hline
AIM-7-50-6-16&9.2&4.6&403&138&50&66\\\hline
AIM-7-50-6-21&13.7&5.8&521&181&58&65\\\hline
AIM-7-50-6-6&3.4&1.5&150&52&56&65\\\hline
AIM-7-50-9-1&0.5&0.3&26&14&40&46\\\hline
AIM-7-50-9-11&6.8&4.8&276&216&29&22\\\hline
AIM-7-50-9-16&9.8&6.9&397&323&30&19\\\hline
AIM-7-50-9-21&12.1&9.9&512&419&18&18\\\hline
AIM-7-50-9-6&3.4&2.8&142&114&18&20\\\hline
AIM-7-100-12-11&18.7&9.8&557&191&48&66\\\hline
AIM-7-100-12-1&1.7&0.8&52&17&53&67\\\hline
AIM-7-100-12-16&28.2&14.3&807&278&49&66\\\hline
AIM-7-100-12-21&41.8&16.3&1043&364&61&65\\\hline
AIM-7-100-12-6&11.4&5.2&299&103&54&66\\\hline
AIM-7-100-3-11&21.4&9.6&532&191&55&64\\\hline
AIM-7-100-3-1&1.7&0.8&50&17&53&66\\\hline
AIM-7-100-3-16&30.3&12.0&773&278&60&64\\\hline
AIM-7-100-3-21&35.5&15.7&1016&366&56&64\\\hline
AIM-7-100-3-6&12.1&5.4&291&104&55&64\\\hline
AIM-7-100-6-11&20.4&9.6&531&187&53&65\\\hline
AIM-7-100-6-1&1.6&0.8&50&17&50&66\\\hline
AIM-7-100-6-16&29.8&13.0&770&272&56&65\\\hline
AIM-7-100-6-21&39.6&15.0&1014&358&62&65\\\hline
AIM-7-100-6-6&11.6&4.7&291&102&59&65\\\hline
AIM-7-100-9-11&19.9&9.1&555&194&54&65\\\hline
AIM-7-100-9-1&1.8&0.9&52&17&50&67\\\hline
AIM-7-100-9-16&28.1&12.5&797&282&56&65\\\hline
AIM-7-100-9-21&40.7&16.7&1052&370&59&65\\\hline
AIM-7-100-9-6&10.8&5.3&296&105&51&65\\\hline
AIM-7-150-12-11&42.2&31.6&807&564&25&30\\\hline
AIM-7-150-12-1&3.7&2.0&76&30&46&61\\\hline
AIM-7-150-12-16&61.5&47.6&1177&889&23&24\\\hline
AIM-7-150-12-21&78.5&55.4&1542&1167&29&24\\\hline
AIM-7-150-12-6&25.2&15.4&441&243&39&45\\\hline
AIM-7-150-3-11&43.0&21.7&786&357&50&55\\\hline
AIM-7-150-3-1&3.4&1.7&74&28&50&62\\\hline
AIM-7-150-3-16&59.2&29.9&1140&561&49&51\\\hline
AIM-7-150-3-21&71.3&41.6&1499&793&42&47\\\hline
AIM-7-150-3-6&24.4&12.0&429&179&51&58\\\hline
AIM-7-150-6-11&44.1&26.3&784&420&40&46\\\hline
AIM-7-150-6-1&3.4&1.8&74&27&47&64\\\hline
AIM-7-150-6-16&60.2&41.6&1140&696&31&39\\\hline
AIM-7-150-6-21&78.8&52.4&1494&1027&34&31\\\hline
AIM-7-150-6-6&24.3&12.8&429&197&47&54\\\hline
AIM-7-150-9-11&41.9&27.8&797&492&34&38\\\hline
AIM-7-150-9-1&3.6&1.9&75&29&47&61\\\hline
AIM-7-150-9-16&57.2&44.1&1155&841&23&27\\\hline
AIM-7-150-9-21&81.4&53.6&1521&1143&34&25\\\hline
AIM-7-150-9-6&21.4&13.5&436&221&37&49\\\hline
AIM-9-50-12-1&1.1&0.4&48&13&64&73\\\hline
AIM-9-50-12-11&15.3&5.3&484&145&65&70\\\hline
AIM-9-50-12-16&19.6&6.7&701&211&66&70\\\hline
AIM-9-50-12-21&24.6&8.4&918&276&66&70\\\hline
AIM-9-50-12-6&7.7&3.0&267&79&61&70\\\hline
AIM-9-50-3-1&1.1&0.5&41&18&55&56\\\hline
AIM-9-50-3-11&13.2&7.5&424&251&43&41\\\hline
AIM-9-50-3-16&16.7&13.2&614&427&21&30\\\hline
AIM-9-50-3-21&22.0&14.9&808&579&32&28\\\hline
AIM-9-50-3-6&7.5&3.7&233&114&51&51\\\hline
AIM-9-50-6-11&14.4&5.0&445&142&65&68\\\hline
AIM-9-50-6-1&1.2&0.4&43&13&67&70\\\hline
AIM-9-50-6-16&21.3&7.8&645&206&63&68\\\hline
AIM-9-50-6-21&27.1&10.1&835&269&63&68\\\hline
AIM-9-50-6-6&7.0&2.8&241&77&60&68\\\hline
AIM-9-50-9-1&1.1&0.6&43&22&45&49\\\hline
AIM-9-50-9-11&14.1&10.7&442&328&24&26\\\hline
AIM-9-50-9-16&18.5&15.0&636&490&19&23\\\hline
AIM-9-50-9-21&27.6&18.2&823&637&34&23\\\hline
AIM-9-50-9-6&7.0&5.4&231&174&23&25\\\hline
AIM-9-100-12-11&41.5&17.3&891&282&58&68\\\hline
AIM-9-100-12-1&3.8&1.6&87&26&58&70\\\hline
AIM-9-100-12-16&62.8&25.2&1290&411&60&68\\\hline
AIM-9-100-12-21&78.9&28.6&1671&536&64&68\\\hline
AIM-9-100-12-6&23.1&9.6&482&153&58&68\\\hline
AIM-9-100-3-11&42.2&16.6&849&284&61&67\\\hline
AIM-9-100-3-1&3.4&1.4&83&26&59&69\\\hline
AIM-9-100-3-16&58.1&21.9&1232&413&62&66\\\hline
AIM-9-100-3-21&78.0&28.8&1618&542&63&67\\\hline
AIM-9-100-3-6&24.2&10.1&466&155&58&67\\\hline
AIM-9-100-6-11&43.8&17.9&848&279&59&67\\\hline
AIM-9-100-6-1&3.6&1.5&83&26&58&69\\\hline
AIM-9-100-6-16&60.5&23.8&1228&405&61&67\\\hline
AIM-9-100-6-21&78.4&28.0&1616&532&64&67\\\hline
AIM-9-100-6-6&23.0&9.3&466&152&60&67\\\hline
AIM-9-100-9-11&43.2&17.7&888&287&59&68\\\hline
AIM-9-100-9-1&3.7&1.6&87&26&57&70\\\hline
AIM-9-100-9-16&61.8&22.9&1278&416&63&67\\\hline
AIM-9-100-9-21&85.7&30.8&1683&547&64&67\\\hline
AIM-9-100-9-6&24.0&9.5&478&156&60&67\\\hline
AIM-9-150-12-11&88.0&64.3&1290&841&27&35\\\hline
AIM-9-150-12-16&118.8&93.3&1878&1324&21&29\\\hline
AIM-9-150-12-1&6.3&3.8&126&46&40&63\\\hline
AIM-9-150-12-21&133.8&122.6&2460&1737&8&29\\\hline
AIM-9-150-12-6&47.5&29.1&708&366&39&48\\\hline
AIM-9-150-3-11&81.0&43.1&1254&531&47&58\\\hline
AIM-9-150-3-16&100.6&57.6&1816&833&43&54\\\hline
AIM-9-150-3-1&6.7&3.1&122&43&54&65\\\hline
AIM-9-150-3-21&122.7&82.4&2386&1176&33&51\\\hline
AIM-9-150-3-6&44.2&21.5&687&267&51&61\\\hline
AIM-9-150-6-11&74.7&47.4&1251&634&37&49\\\hline
AIM-9-150-6-16&99.0&75.1&1817&1053&24&42\\\hline
AIM-9-150-6-1&7.0&3.2&122&42&54&66\\\hline
AIM-9-150-6-21&129.0&109.2&2380&1554&15&35\\\hline
AIM-9-150-6-6&42.8&23.4&686&297&45&57\\\hline
AIM-9-150-9-11&81.4&56.6&1272&734&30&42\\\hline
AIM-9-150-9-16&117.5&91.4&1843&1250&22&32\\\hline
AIM-9-150-9-1&7.4&3.4&124&44&54&65\\\hline
AIM-9-150-9-21&138.5&121.6&2423&1696&12&30\\\hline
AIM-9-150-9-6&44.9&19.4&699&331&57&53\\\hline
AIM-11-50-12-11&27.3&8.5&711&201&69&72\\\hline
AIM-11-50-12-1&2.0&0.7&72&18&65&75\\\hline
AIM-11-50-12-16&37.6&11.6&1028&293&69&71\\\hline
AIM-11-50-12-21&46.6&13.6&1346&384&71&71\\\hline
AIM-11-50-12-6&14.4&4.7&393&110&67&72\\\hline
AIM-11-50-3-11&23.4&12.6&619&360&46&42\\\hline
AIM-11-50-3-1&1.8&0.9&62&26&50&58\\\hline
AIM-11-50-3-16&32.5&19.2&897&615&41&31\\\hline
AIM-11-50-3-21&43.2&25.1&1178&834&42&29\\\hline
AIM-11-50-3-6&13.2&6.3&341&162&52&52\\\hline
AIM-11-50-6-11&26.0&8.5&651&197&67&70\\\hline
AIM-11-50-6-1&2.1&0.6&65&18&71&72\\\hline
AIM-11-50-6-16&38.2&13.6&943&286&64&70\\\hline
AIM-11-50-6-21&46.0&15.5&1223&374&66&69\\\hline
AIM-11-50-6-6&13.0&4.5&354&107&65&70\\\hline
AIM-11-50-9-11&24.5&16.5&648&475&33&27\\\hline
AIM-11-50-9-1&2.0&1.0&65&33&50&49\\\hline
AIM-11-50-9-16&36.4&28.1&932&710&23&24\\\hline
AIM-11-50-9-21&48.1&29.4&1208&924&39&24\\\hline
AIM-11-50-9-6&11.9&9.4&342&255&21&25\\\hline
AIM-11-100-12-11&79.5&28.6&1302&393&64&70\\\hline
AIM-11-100-12-16&115.8&43.4&1885&570&63&70\\\hline
AIM-11-100-12-1&6.7&2.6&130&36&61&72\\\hline
AIM-11-100-12-21&148.6&49.6&2446&745&67&70\\\hline
AIM-11-100-12-6&41.5&15.3&708&214&63&70\\\hline
AIM-11-100-3-11&70.9&27.3&1240&395&61&68\\\hline
AIM-11-100-3-1&5.9&2.3&124&37&61&70\\\hline
AIM-11-100-3-16&103.7&37.8&1797&574&64&68\\\hline
AIM-11-100-3-21&132.4&51.7&2359&753&61&68\\\hline
AIM-11-100-3-6&42.2&16.5&682&216&61&68\\\hline
AIM-11-100-6-11&75.7&30.4&1239&388&60&69\\\hline
AIM-11-100-6-16&107.8&40.9&1793&563&62&69\\\hline
AIM-11-100-6-1&6.2&2.4&123&37&61&70\\\hline
AIM-11-100-6-21&138.4&50.3&2356&739&64&69\\\hline
AIM-11-100-6-6&41.8&15.3&682&212&63&69\\\hline
AIM-11-100-9-11&79.2&30.5&1299&400&61&69\\\hline
AIM-11-100-9-16&111.2&42.8&1870&579&62&69\\\hline
AIM-11-100-9-1&6.6&2.8&130&37&58&72\\\hline
AIM-11-100-9-21&152.7&58.5&2461&761&62&69\\\hline
AIM-11-100-9-6&43.6&15.7&703&217&64&69\\\hline
AIM-11-150-12-11&161.2&111.0&1885&1212&31&36\\\hline
AIM-11-150-12-1&13.5&6.3&188&66&53&65\\\hline
AIM-11-150-12-16&218.6&161.3&2742&1912&26&30\\\hline
AIM-11-150-12-21&285.0&194.2&3590&2508&32&30\\\hline
AIM-11-150-12-6&89.1&49.0&1036&523&45&50\\\hline
AIM-11-150-3-11&144.6&71.1&1830&750&51&59\\\hline
AIM-11-150-3-1&12.2&5.2&182&61&57&66\\\hline
AIM-11-150-3-16&206.1&102.3&2649&1181&50&55\\\hline
AIM-11-150-3-21&276.0&133.9&3477&1672&51&52\\\hline
AIM-11-150-3-6&77.6&37.0&1004&376&52&63\\\hline
AIM-11-150-6-11&152.7&85.9&1826&901&44&51\\\hline
AIM-11-150-6-1&13.2&5.7&182&61&57&66\\\hline
AIM-11-150-6-16&222.9&128.6&2650&1503&42&43\\\hline
AIM-11-150-6-21&276.6&173.1&3470&2226&37&36\\\hline
AIM-11-150-6-6&83.1&41.3&1003&420&50&58\\\hline
AIM-11-150-9-11&152.7&89.9&1858&1052&41&43\\\hline
AIM-11-150-9-1&12.8&5.9&185&63&54&66\\\hline
AIM-11-150-9-16&216.8&143.9&2690&1803&34&33\\\hline
AIM-11-150-9-21&270.4&180.4&3534&2447&33&31\\\hline
AIM-11-150-9-6&84.6&43.9&1022&471&48&54\\\hline
AIM-13-50-12-11&43.6&13.3&980&267&69&73\\\hline
AIM-13-50-12-1&3.4&1.0&100&25&71&75\\\hline
AIM-13-50-12-16&63.1&19.3&1418&388&69&73\\\hline
AIM-13-50-12-21&81.4&24.7&1856&509&70&73\\\hline
AIM-13-50-12-6&23.5&7.2&542&146&69&73\\\hline
AIM-13-50-3-11&37.3&22.6&851&488&39&43\\\hline
AIM-13-50-3-1&3.0&1.4&86&36&53&58\\\hline
AIM-13-50-3-16&52.3&38.0&1232&837&27&32\\\hline
AIM-13-50-3-21&70.8&49.9&1618&1135&30&30\\\hline
AIM-13-50-3-6&21.1&10.2&469&219&52&53\\\hline
AIM-13-50-6-11&40.8&13.1&896&261&68&71\\\hline
AIM-13-50-6-1&3.4&1.2&91&25&65&73\\\hline
AIM-13-50-6-16&51.6&22.9&1297&379&56&71\\\hline
AIM-13-50-6-21&73.4&28.8&1684&496&61&71\\\hline
AIM-13-50-6-6&21.6&6.9&489&143&68&71\\\hline
AIM-13-50-9-11&40.0&29.9&892&648&25&27\\\hline
AIM-13-50-9-1&3.3&1.7&91&45&48&51\\\hline
AIM-13-50-9-16&53.3&44.2&1284&970&17&24\\\hline
AIM-13-50-9-21&75.4&54.0&1666&1264&28&24\\\hline
AIM-13-50-9-6&18.7&15.7&474&351&16&26\\\hline
AIM-13-100-12-1&10.8&3.7&182&49&66&73\\\hline
AIM-13-100-12-11&121.6&40.1&1792&520&67&71\\\hline
AIM-13-100-12-16&179.3&68.4&2593&756&62&71\\\hline
AIM-13-100-12-21&233.9&89.7&3368&988&62&71\\\hline
AIM-13-100-12-6&68.2&23.9&977&284&65&71\\\hline
AIM-13-100-3-11&116.5&44.9&1704&524&61&69\\\hline
AIM-13-100-3-16&173.7&64.0&2469&761&63&69\\\hline
AIM-13-100-3-1&9.9&3.6&173&50&64&71\\\hline
AIM-13-100-3-21&202.3&76.4&3239&998&62&69\\\hline
AIM-13-100-3-6&67.9&25.4&939&288&63&69\\\hline
AIM-13-100-6-1&10.0&3.8&172&50&62&71\\\hline
AIM-13-100-6-11&117.9&46.6&1702&514&60&70\\\hline
AIM-13-100-6-16&173.9&63.2&2464&746&64&70\\\hline
AIM-13-100-6-21&212.8&76.6&3235&979&64&70\\\hline
AIM-13-100-6-6&67.3&23.1&938&282&66&70\\\hline
AIM-13-100-9-1&10.7&4.2&182&51&61&72\\\hline
AIM-13-100-9-11&127.1&46.5&1788&531&63&70\\\hline
AIM-13-100-9-16&175.2&65.8&2575&769&62&70\\\hline
AIM-13-100-9-21&228.3&88.1&3386&1009&61&70\\\hline
AIM-13-100-9-6&71.0&23.6&971&289&67&70\\\hline
AIM-13-150-12-11&233.4&163.1&2593&1649&30&36\\\hline
AIM-13-150-12-1&20.4&9.6&263&91&53&65\\\hline
AIM-13-150-12-16&313.8&242.5&3768&2604&23&31\\\hline
AIM-13-150-12-21&423.6&291.2&4932&3416&31&31\\\hline
AIM-13-150-12-6&138.6&73.1&1428&709&47&50\\\hline
AIM-13-150-3-11&210.7&99.4&2513&1006&53&60\\\hline
AIM-13-150-3-1&19.9&8.2&254&83&59&67\\\hline
AIM-13-150-3-16&316.1&146.5&3638&1587&54&56\\\hline
AIM-13-150-3-21&403.5&193.1&4772&2253&52&53\\\hline
AIM-13-150-3-6&132.2&53.9&1382&503&59&64\\\hline
AIM-13-150-6-11&219.6&126.4&2509&1215&42&52\\\hline
AIM-13-150-6-1&20.1&8.5&254&82&58&68\\\hline
AIM-13-150-6-16&298.2&190.8&3639&2032&36&44\\\hline
AIM-13-150-6-21&422.5&269.2&4764&3016&36&37\\\hline
AIM-13-150-6-6&136.5&61.3&1381&565&55&59\\\hline
AIM-13-150-9-11&222.5&137.0&2554&1427&38&44\\\hline
AIM-13-150-9-1&20.9&8.9&258&86&57&67\\\hline
AIM-13-150-9-16&337.0&219.9&3696&2454&35&34\\\hline
AIM-13-150-9-21&408.0&294.1&4853&3331&28&31\\\hline
AIM-13-150-9-6&133.8&59.4&1407&636&56&55\\\hline
consVprod2-2&0.2&0.2&113&73&0&35\\\hline
consVprod2-3&1.9&0.1&1078&65&95&94\\\hline
consVprod2-4&0.2&0.1&173&70&50&60\\\hline
consVprod2-5&5.4&2.8&3952&2099&48&47\\\hline
consVprod2-6&7.7&4.9&6276&3473&36&45\\\hline
consVprod2-7&9.7&5.5&8595&4523&43&47\\\hline
consVprod2-8&4.7&3.7&5790&3922&21&32\\\hline
consVprod3-2&405.3&244.7&197581&128078&40&35\\\hline
consVprod3-3&2013.0&1110.0&876883&473159&45&46\\\hline
consVprod3-4&2133.0&1484.0&1413182&964672&30&32\\\hline
consVprod3-5&3243.0&1910.0&2497931&1318165&41&47\\\hline
consVprod3-6&TO&TO&TO&TO&-&-\\\hline
consVprod3-7&TO&TO&TO&TO&-&-\\\hline
consVprod3-8&TO&TO&TO&TO&-&-\\\hline
consVprod4-2&12230.0&1975.0&1775373&784628&84&56\\\hline
consVprod4-3&TO&7039.0&TO&1865954&-&-\\\hline
consVprod4-4&TO&TO&TO&TO&-&-\\\hline
consVprod4-5&4.4&0.1&3924&35&98&99\\\hline
consVprod4-6&TO&TO&TO&TO&-&-\\\hline
consVprod4-7&TO&TO&TO&TO&-&-\\\hline
consVprod4-8&TO&TO&TO&TO&-&-\\\hline
consVprod5-2&TO&TO&TO&TO&-&-\\\hline
consVprod5-3&TO&TO&TO&TO&-&-\\\hline
consVprod5-4&TO&TO&TO&TO&-&-\\\hline
consVprod5-5&TO&TO&TO&TO&-&-\\\hline
consVprod5-6&TO&TO&TO&TO&-&-\\\hline
consVprod5-7&TO&TO&TO&TO&-&-\\\hline
consVprod5-8&TO&TO&TO&TO&-&-\\\hline
consVprod6-2&TO&TO&TO&TO&-&-\\\hline
consVprod6-3&TO&TO&TO&TO&-&-\\\hline
consVprod6-4&406.5&0.5&123497&142&100&100\\\hline
consVprod6-5&TO&TO&TO&TO&-&-\\\hline
consVprod6-6&TO&TO&TO&TO&-&-\\\hline
consVprod6-7&TO&TO&TO&TO&-&-\\\hline
consVprod6-8&TO&TO&TO&TO&-&-\\\hline
consVprod7-2&0.3&0.0&149&0&100&100\\\hline
consVprod7-3&249.7&0.6&135516&135&100&100\\\hline
consVprod7-4&TO&TO&TO&TO&-&-\\\hline
consVprod7-5&TO&TO&TO&TO&-&-\\\hline
consVprod7-6&TO&TO&TO&TO&-&-\\\hline
consVprod7-7&TO&TO&TO&TO&-&-\\\hline
consVprod7-8&TO&TO&TO&TO&-&-\\\hline
consVprod8-2&TO&TO&TO&TO&-&-\\\hline
consVprod8-3&TO&TO&TO&TO&-&-\\\hline
consVprod8-4&TO&TO&TO&TO&-&-\\\hline
consVprod8-5&TO&TO&TO&TO&-&-\\\hline
consVprod8-6&TO&TO&TO&TO&-&-\\\hline
consVprod8-7&TO&TO&TO&TO&-&-\\\hline
consVprod8-8&TO&TO&TO&TO&-&-\\\hline
Lyngby2&3292.0&215.5&1511749&87214&93&94\\\hline
Lyngby3&TO&TO&TO&TO&-&-\\\hline
Lyngby4&TO&TO&TO&TO&-&-\\\hline
Lyngby5&TO&TO&TO&TO&-&-\\\hline
LyngbySmall2&3.4&1.0&1803&444&71&75\\\hline
LyngbySmall3&23.1&26.1&11473&10701&-13&7\\\hline
LyngbySmall4&144.3&193.3&65371&70008&-34&-7\\\hline
manf-workflow-4&0.2&0.0&68&1&100&99\\\hline
manf-workflow-5&0.3&0.0&134&1&100&99\\\hline
manf-workflow-6&0.6&0.0&232&2&100&99\\\hline
manf-workflow-7&1.1&0.0&368&2&100&99\\\hline
manf-workflow-8&1.8&0.0&550&2&100&100\\\hline
manf-workflow-9&2.6&0.0&785&2&100&100\\\hline
manf-workflow-10&3.9&0.0&1077&2&100&100\\\hline
manf-workflow-11&5.5&0.0&1435&3&100&100\\\hline
manf-workflow-12&7.3&0.0&1864&3&100&100\\\hline
manf-workflow-13&9.7&0.0&2371&3&100&100\\\hline
manf-workflow-14&12.6&0.0&2963&3&100&100\\\hline
manf-workflow-15&16.4&0.0&3646&3&100&100\\\hline
manf-workflow-20&46.4&0.0&8657&4&100&100\\\hline
manf-workflow-25&111.8&0.0&16926&5&100&100\\\hline
manf-workflow-30&227.8&0.1&29269&7&100&100\\\hline
manf-workflow-35&420.3&0.1&46501&8&100&100\\\hline
manf-workflow-40&735.3&0.2&69439&9&100&100\\\hline
manf-workflow-45&1238.0&0.2&98899&10&100&100\\\hline
manf-workflow-50&1952.0&0.2&135697&11&100&100\\\hline
manf-workflow-60&4417.0&0.3&234570&13&100&100\\\hline
manf-workflow-70&TO&0.3&TO&15&-&-\\\hline
manf-workflow-80&TO&0.6&TO&17&-&-\\\hline
manf-workflow-90&TO&0.7&TO&19&-&-\\\hline
manf-workflow-100&TO&0.9&TO&21&-&-\\\hline

nim3-10500&0.4&0.3&179&116&25&35\\\hline
nim3-11500&0.4&0.4&196&127&0&35\\\hline
nim3-12500&0.4&0.4&213&138&0&35\\\hline
nim3-13500&0.4&0.4&230&149&0&35\\\hline
nim3-14500&0.5&0.5&247&160&0&35\\\hline
nim3-1500&0.1&0.1&26&17&0&35\\\hline
nim3-15500&0.6&0.4&264&171&33&35\\\hline
nim3-16500&0.6&0.6&281&182&0&35\\\hline
nim3-17500&0.5&0.6&298&193&-20&35\\\hline
nim3-18500&0.7&0.4&315&204&43&35\\\hline
nim3-19500&0.7&0.7&332&215&0&35\\\hline
nim3-20500&0.7&0.7&349&226&0&35\\\hline
nim3-21500&0.7&0.7&366&237&0&35\\\hline
nim3-22500&0.7&0.7&383&248&0&35\\\hline
nim3-23500&0.9&0.7&400&259&22&35\\\hline
nim3-24500&0.9&0.7&417&270&22&35\\\hline
nim3-2500&0.1&0.1&43&28&0&35\\\hline
nim3-25500&1.0&0.8&434&281&20&35\\\hline
nim3-26500&0.9&0.8&451&292&11&35\\\hline
nim3-27500&1.0&0.9&468&303&10&35\\\hline
nim3-28500&1.1&0.9&485&314&18&35\\\hline
nim3-29500&1.1&0.8&502&325&27&35\\\hline
nim3-30500&1.2&0.9&519&336&25&35\\\hline
nim3-31500&1.2&0.8&536&347&33&35\\\hline
nim3-32500&1.3&0.9&553&358&31&35\\\hline
nim3-33500&1.3&1.1&570&369&15&35\\\hline
nim3-34500&1.4&1.1&587&380&21&35\\\hline
nim3-3500&0.1&0.1&60&39&0&35\\\hline
nim3-35500&1.1&1.0&604&391&9&35\\\hline
nim3-36500&1.5&1.2&621&402&20&35\\\hline
nim3-37500&1.5&1.0&638&413&33&35\\\hline
nim3-38500&1.6&1.0&655&424&38&35\\\hline
nim3-39500&1.6&1.3&672&435&19&35\\\hline
nim3-40500&1.7&1.3&689&446&24&35\\\hline
nim3-41500&1.5&1.4&706&457&7&35\\\hline
nim3-42500&1.4&1.5&723&468&-7&35\\\hline
nim3-43500&1.8&1.5&740&479&17&35\\\hline
nim3-44500&1.6&1.3&757&490&19&35\\\hline
nim3-4500&0.2&0.1&77&50&50&35\\\hline
nim3-45500&1.8&1.7&774&501&6&35\\\hline
nim3-46500&1.8&1.7&791&512&6&35\\\hline
nim3-47500&2.0&1.8&808&523&10&35\\\hline
nim3-48500&2.2&1.8&825&534&18&35\\\hline
nim3-49500&2.2&1.9&842&545&14&35\\\hline
nim3-500&0.0&0.0&9&6&0&33\\\hline
nim3-5500&0.2&0.1&94&61&50&35\\\hline
nim3-6500&0.2&0.2&111&72&0&35\\\hline
nim3-7500&0.3&0.2&128&83&33&35\\\hline
nim3-8500&0.3&0.3&145&94&0&35\\\hline
nim3-9500&0.3&0.3&162&105&0&35\\\hline
nim4-10500&0.7&0.3&448&153&57&66\\\hline
nim4-11500&0.7&0.4&491&167&43&66\\\hline
nim4-12500&0.9&0.5&533&182&44&66\\\hline
nim4-13500&1.0&0.6&576&196&40&66\\\hline
nim4-14500&1.0&0.5&618&211&50&66\\\hline
nim4-1500&0.1&0.1&66&22&0&67\\\hline
nim4-15500&1.0&0.7&661&225&30&66\\\hline
nim4-16500&1.3&0.7&703&240&46&66\\\hline
nim4-17500&1.4&0.7&746&254&50&66\\\hline
nim4-18500&1.4&0.9&788&269&36&66\\\hline
nim4-19500&1.1&0.8&831&283&27&66\\\hline
nim4-20500&1.3&0.9&873&298&31&66\\\hline
nim4-21500&1.6&0.9&916&312&44&66\\\hline
nim4-22500&1.7&1.0&958&327&41&66\\\hline
nim4-23500&1.6&1.0&1001&341&38&66\\\hline
nim4-24500&1.6&0.9&1043&356&44&66\\\hline
nim4-2500&0.2&0.1&108&37&50&66\\\hline
nim4-25500&2.1&1.2&1086&370&43&66\\\hline
nim4-26500&2.1&1.3&1128&385&38&66\\\hline
nim4-27500&2.1&1.0&1171&399&52&66\\\hline
nim4-28500&2.2&1.3&1213&414&41&66\\\hline
nim4-29500&2.1&1.4&1256&428&33&66\\\hline
nim4-30500&2.4&1.3&1298&443&46&66\\\hline
nim4-31500&2.1&1.3&1341&457&38&66\\\hline
nim4-32500&2.1&1.6&1383&472&24&66\\\hline
nim4-33500&2.7&1.4&1426&486&48&66\\\hline
nim4-34500&2.4&1.5&1468&501&38&66\\\hline
nim4-3500&0.2&0.1&151&51&50&66\\\hline
nim4-35500&3.0&1.6&1511&515&47&66\\\hline
nim4-36500&3.2&1.7&1553&530&47&66\\\hline
nim4-37500&3.2&1.6&1596&544&50&66\\\hline
nim4-38500&3.3&1.6&1638&559&52&66\\\hline
nim4-39500&3.3&1.8&1681&573&45&66\\\hline
nim4-40500&3.4&2.1&1723&588&38&66\\\hline
nim4-41500&3.6&2.1&1766&602&42&66\\\hline
nim4-42500&3.4&2.2&1808&617&35&66\\\hline
nim4-43500&3.8&2.2&1851&631&42&66\\\hline
nim4-44500&3.9&2.2&1893&646&44&66\\\hline
nim4-4500&0.3&0.2&193&66&33&66\\\hline
nim4-45500&4.0&2.0&1936&660&50&66\\\hline
nim4-46500&4.1&2.4&1978&675&41&66\\\hline
nim4-47500&4.3&2.1&2021&689&51&66\\\hline
nim4-48500&3.7&2.1&2063&704&43&66\\\hline
nim4-49500&4.2&2.6&2106&718&38&66\\\hline
nim4-500&0.1&0.0&23&8&100&65\\\hline
nim4-5500&0.4&0.2&236&80&50&66\\\hline
nim4-6500&0.4&0.2&278&95&50&66\\\hline
nim4-7500&0.5&0.3&321&109&40&66\\\hline
nim4-8500&0.6&0.4&363&124&33&66\\\hline
nim4-9500&0.6&0.4&406&138&33&66\\\hline
nim5-10500&1.6&0.5&1076&190&69&82\\\hline
nim5-11500&1.7&0.7&1178&208&59&82\\\hline
nim5-12500&1.9&0.7&1280&226&63&82\\\hline
nim5-13500&2.0&0.6&1382&244&70&82\\\hline
nim5-14500&1.9&0.7&1484&262&63&82\\\hline
nim5-1500&0.3&0.1&158&28&67&82\\\hline
nim5-15500&2.1&0.9&1586&280&57&82\\\hline
nim5-16500&2.5&0.9&1688&298&64&82\\\hline
nim5-17500&2.8&1.0&1790&316&64&82\\\hline
nim5-18500&2.9&1.1&1892&334&62&82\\\hline
nim5-19500&3.0&1.2&1994&352&60&82\\\hline
nim5-20500&3.1&1.2&2096&370&61&82\\\hline
nim5-21500&39.8&1.3&2198&388&97&82\\\hline
nim5-22500&3.5&1.3&2300&406&63&82\\\hline
nim5-23500&3.7&1.4&2402&424&62&82\\\hline
nim5-24500&3.9&1.5&2504&442&62&82\\\hline
nim5-2500&0.3&0.2&260&46&33&82\\\hline
nim5-25500&3.7&1.7&2606&460&54&82\\\hline
nim5-26500&3.5&1.7&2708&478&51&82\\\hline
nim5-27500&4.5&1.8&2810&496&60&82\\\hline
nim5-28500&4.6&1.8&2912&514&61&82\\\hline
nim5-29500&4.8&1.9&3014&532&60&82\\\hline
nim5-30500&5.0&1.9&3116&550&62&82\\\hline
nim5-31500&5.1&2.0&3218&568&61&82\\\hline
nim5-32500&4.8&2.0&3320&586&58&82\\\hline
nim5-33500&5.7&2.0&3422&604&65&82\\\hline
nim5-34500&5.9&2.2&3524&622&63&82\\\hline
nim5-3500&0.5&0.2&362&64&60&82\\\hline
nim5-35500&5.1&2.2&3626&640&57&82\\\hline
nim5-36500&6.3&2.3&3728&658&63&82\\\hline
nim5-37500&6.6&2.4&3830&676&64&82\\\hline
nim5-38500&6.6&2.5&3932&694&62&82\\\hline
nim5-39500&6.7&2.4&4034&712&64&82\\\hline
nim5-40500&6.9&2.5&4136&730&64&82\\\hline
nim5-41500&7.2&2.6&4238&748&64&82\\\hline
nim5-42500&7.4&2.5&4340&766&66&82\\\hline
nim5-43500&7.6&3.0&4442&784&61&82\\\hline
nim5-44500&8.1&3.1&4544&802&62&82\\\hline
nim5-4500&0.5&0.2&464&82&60&82\\\hline
nim5-45500&7.4&2.8&4646&820&62&82\\\hline
nim5-46500&6.8&2.5&4748&838&63&82\\\hline
nim5-47500&8.7&3.2&4850&856&63&82\\\hline
nim5-48500&8.8&3.4&4952&874&61&82\\\hline
nim5-49500&9.2&3.4&5054&892&63&82\\\hline
nim5-500&0.1&0.0&56&10&100&82\\\hline
nim5-5500&0.8&0.3&566&100&62&82\\\hline
nim5-6500&0.9&0.3&668&118&67&82\\\hline
nim5-7500&1.0&0.5&770&136&50&82\\\hline
nim5-8500&1.2&0.5&872&154&58&82\\\hline
nim5-9500&1.4&0.5&974&172&64&82\\\hline
nim6-10500&3.0&0.7&2478&235&77&91\\\hline
nim6-11500&2.9&0.8&2713&257&72&91\\\hline
nim6-12500&3.7&0.9&2948&279&76&91\\\hline
nim6-13500&3.7&1.0&3183&301&73&91\\\hline
nim6-14500&4.4&1.0&3418&324&77&91\\\hline
nim6-1500&0.5&0.1&363&34&80&91\\\hline
nim6-15500&4.7&1.1&3653&346&77&91\\\hline
nim6-16500&5.0&1.2&3888&368&76&91\\\hline
nim6-17500&4.9&1.2&4123&390&76&91\\\hline
nim6-18500&5.3&1.3&4358&413&75&91\\\hline
nim6-19500&4.7&1.3&4593&435&72&91\\\hline
nim6-20500&6.0&1.4&4828&457&77&91\\\hline
nim6-21500&5.9&1.4&5063&479&76&91\\\hline
nim6-22500&6.9&1.7&5298&502&75&91\\\hline
nim6-23500&7.2&1.6&5533&524&78&91\\\hline
nim6-24500&6.9&1.5&5768&546&78&91\\\hline
nim6-2500&0.7&0.2&598&57&71&90\\\hline
nim6-25500&6.4&1.5&6003&568&77&91\\\hline
nim6-26500&8.1&1.7&6238&591&79&91\\\hline
nim6-27500&8.3&2.0&6473&613&76&91\\\hline
nim6-28500&9.0&2.0&6708&635&78&91\\\hline
nim6-29500&8.2&2.0&6943&657&76&91\\\hline
nim6-30500&9.4&1.7&7178&680&82&91\\\hline
nim6-31500&9.8&2.3&7413&702&77&91\\\hline
nim6-32500&10.2&2.4&7648&724&76&91\\\hline
nim6-33500&11.0&2.5&7883&746&77&91\\\hline
nim6-34500&10.9&2.6&8118&769&76&91\\\hline
nim6-3500&1.1&0.2&833&79&82&91\\\hline
nim6-35500&9.4&2.4&8353&791&74&91\\\hline
nim6-36500&11.8&2.8&8588&813&76&91\\\hline
nim6-37500&12.1&2.8&8823&835&77&91\\\hline
nim6-38500&12.5&3.0&9058&858&76&91\\\hline
nim6-39500&12.7&3.0&9293&880&76&91\\\hline
nim6-40500&13.1&3.1&9528&902&76&91\\\hline
nim6-41500&13.2&3.1&9763&924&77&91\\\hline
nim6-42500&13.6&3.1&9998&947&77&91\\\hline
nim6-43500&11.8&3.2&10233&969&73&91\\\hline
nim6-44500&14.6&3.5&10468&991&76&91\\\hline
nim6-4500&1.3&0.3&1068&101&77&91\\\hline
nim6-45500&14.9&3.5&10703&1013&77&91\\\hline
nim6-46500&14.4&3.1&10938&1036&78&91\\\hline
nim6-47500&16.0&3.3&11173&1058&79&91\\\hline
nim6-48500&14.5&3.7&11408&1080&74&91\\\hline
nim6-49500&16.7&3.7&11643&1102&78&91\\\hline
nim6-500&0.2&0.0&128&12&100&91\\\hline
nim6-5500&1.6&0.3&1303&123&81&91\\\hline
nim6-6500&2.0&0.5&1538&146&75&91\\\hline
nim6-7500&1.9&0.4&1773&168&79&91\\\hline
nim6-8500&2.7&0.6&2008&190&78&91\\\hline
nim6-9500&2.9&0.7&2243&212&76&91\\\hline
nim7-10500&6.7&0.7&5117&247&90&95\\\hline
nim7-11500&7.0&0.9&5602&270&87&95\\\hline
nim7-12500&7.7&1.0&6087&294&87&95\\\hline
nim7-13500&6.8&1.1&6572&317&84&95\\\hline
nim7-14500&8.7&0.9&7057&340&90&95\\\hline
nim7-1500&0.9&0.1&750&36&89&95\\\hline
nim7-15500&9.7&1.1&7543&364&89&95\\\hline
nim7-16500&10.2&1.3&8028&387&87&95\\\hline
nim7-17500&10.7&1.3&8513&411&88&95\\\hline
nim7-18500&11.3&1.4&8998&434&88&95\\\hline
nim7-19500&12.1&1.5&9483&457&88&95\\\hline
nim7-20500&10.4&1.6&9969&481&85&95\\\hline
nim7-21500&13.3&1.5&10454&504&89&95\\\hline
nim7-22500&13.9&1.8&10939&528&87&95\\\hline
nim7-23500&14.5&1.8&11424&551&88&95\\\hline
nim7-24500&14.9&2.0&11909&574&87&95\\\hline
nim7-2500&1.6&0.2&1235&60&88&95\\\hline
nim7-25500&15.0&2.0&12395&598&87&95\\\hline
nim7-26500&16.8&2.2&12880&621&87&95\\\hline
nim7-27500&16.8&2.3&13365&645&86&95\\\hline
nim7-28500&18.1&2.4&13850&668&87&95\\\hline
nim7-29500&16.9&2.5&14335&691&85&95\\\hline
nim7-30500&18.6&2.5&14821&715&87&95\\\hline
nim7-31500&20.2&2.5&15306&738&88&95\\\hline
nim7-32500&20.7&2.7&15791&762&87&95\\\hline
nim7-33500&20.9&2.8&16276&785&87&95\\\hline
nim7-34500&19.0&2.9&16761&808&85&95\\\hline
nim7-3500&2.1&0.2&1720&83&90&95\\\hline
nim7-35500&22.0&2.9&17247&832&87&95\\\hline
nim7-36500&23.3&3.0&17732&855&87&95\\\hline
nim7-37500&23.7&3.2&18217&879&86&95\\\hline
nim7-38500&24.1&3.3&18702&902&86&95\\\hline
nim7-39500&25.5&3.3&19187&925&87&95\\\hline
nim7-40500&25.9&3.4&19673&949&87&95\\\hline
nim7-41500&31.9&3.5&20158&972&89&95\\\hline
nim7-42500&28.0&3.3&20643&996&88&95\\\hline
nim7-43500&25.9&3.8&21128&1019&85&95\\\hline
nim7-44500&28.2&3.5&21613&1042&88&95\\\hline
nim7-4500&2.3&0.3&2205&106&87&95\\\hline
nim7-45500&27.9&3.3&22099&1066&88&95\\\hline
nim7-46500&25.3&4.1&22584&1089&84&95\\\hline
nim7-47500&25.1&4.1&23069&1113&84&95\\\hline
nim7-48500&26.6&4.1&23554&1136&85&95\\\hline
nim7-49500&32.7&3.9&24039&1159&88&95\\\hline
nim7-500&0.3&0.0&265&13&100&95\\\hline
nim7-5500&3.4&0.3&2691&130&91&95\\\hline
nim7-6500&3.9&0.5&3176&153&87&95\\\hline
nim7-7500&4.3&0.6&3661&177&86&95\\\hline
nim7-8500&4.7&0.7&4146&200&85&95\\\hline
nim7-9500&5.7&0.6&4631&223&89&95\\\hline
order-workflow-10k&0.9&0.7&320&240&22&25\\\hline
order-workflow-20k&1.8&1.5&640&480&17&25\\\hline
order-workflow-30k&2.9&2.0&960&720&31&25\\\hline
order-workflow-40k&4.0&3.5&1280&960&12&25\\\hline
order-workflow-50k&5.3&4.5&1600&1200&15&25\\\hline
order-workflow-60k&6.6&5.7&1920&1440&14&25\\\hline
order-workflow-70k&7.8&6.6&2240&1680&15&25\\\hline
order-workflow-80k&8.8&7.5&2560&1920&15&25\\\hline
order-workflow-90k&9.8&8.1&2880&2160&17&25\\\hline
order-workflow-100k&11.1&7.8&3200&2400&30&25\\\hline

\hline
\caption{Experiments with and without partial order reduction (POR and NORMAL respectively). The \emph{TO}-notation signifies timout (12 hours).}
\end{longtable}
%}
%\bigskip
%\caption{Experiments with and without partial order reduction (POR and NORMAL respectively).}
%\label{tab:results}
%\end{table}

